Spatiotemporal focusing through a multimode fiber via time-domain wavefront shaping

We shape fs optical pulses and deliver them in a single spatial mode to the input of a multimode fiber. The pulse is shaped in time such that at the output of the multimode fiber an ultrashort pulse appears at a predefined focus. Our result shows how to raster scan an ultrashort pulse at the output of a stiff piece of square-core step-index multimode fiber and in this way the potential for making a nonlinear fluorescent image of the scene behind the fiber, while the connection to the multimode fiber can be established via a thin and flexible single-mode fiber. The experimental results match our numerical simulation well.

==> Spatiotemporal focusing through a multi-mode fiber via time-domain wavefront shaping (revision 2)/tWFS_Velsink2.tex <==
@article{amitonova2016,
  title = {High-resolution wavefront shaping with a photonic crystal fiber for multimode fiber imaging},
  author = {Amitonova, Lyubov V. and Descloux, Adrien and Petschulat, Joerg and Frosz, Michael H. and Ahmed, Goran and Babic, Fehim and Jiang, Xin and Mosk, Allard P. and Russell, Philip St J. and Pinkse, Pepijn W. H.},
  year = {2016},
  month = feb,
  volume = {41},
  pages = {497--500},
  publisher = {{Optical Society of America}},
  issn = {1539-4794},
  doi = {10.1364/OL.41.000497},
  journal = {Opt. Lett.},
  number = {3}
}

@article{amitonova2020,
  title = {Endo-microscopy beyond the {{Abbe}} and {{Nyquist}} limits},
  author = {Amitonova, Lyubov V. and {de Boer}, Johannes F.},
  year = {2020},
  month = may,
  volume = {9},
  pages = {81},
  publisher = {{Nature Publishing Group}},
  issn = {2047-7538},
  doi = {10.1038/s41377-020-0308-x},
  journal = {Light Sci. Appl.},
  number = {1}
}

@article{andresen2013,
  title = {Toward endoscopes with no distal optics: video-rate scanning microscopy through a fiber bundle},
  shorttitle = {Toward endoscopes with no distal optics},
  author = {Andresen, Esben Ravn and Bouwmans, G{\'e}raud and Monneret, Serge and Rigneault, Herv{\'e}},
  year = {2013},
  month = mar,
  volume = {38},
  pages = {609--611},
  publisher = {{Optical Society of America}},
  issn = {1539-4794},
  doi = {10.1364/OL.38.000609},
  journal = {Opt. Lett.},
  number = {5}
}

@article{borhani2018,
  title = {Learning to see through multimode fibers},
  author = {Borhani, Navid and Kakkava, Eirini and Moser, Christophe and Psaltis, Demetri},
  year = {2018},
  month = aug,
  volume = {5},
  pages = {960--966},
  publisher = {{Optical Society of America}},
  issn = {2334-2536},
  doi = {10.1364/OPTICA.5.000960},
  journal = {Optica},
  number = {8}
}

@article{bowlan2006,
  title = {Crossed-beam spectral interferometry: a simple, high-spectral-resolution method for completely characterizing complex ultrashort pulses in real time},
  shorttitle = {Crossed-beam spectral interferometry},
  author = {Bowlan, Pamela and Gabolde, Pablo and Shreenath, Aparna and McGresham, Kristan and Trebino, Rick and Akturk, Selcuk},
  year = {2006},
  month = nov,
  volume = {14},
  pages = {11892--11900},
  publisher = {{Optical Society of America}},
  issn = {1094-4087},
  doi = {10.1364/OE.14.011892},
  journal = {Opt. Express},
  number = {24}
}

@article{cizmar2011,
  title = {Shaping the light transmission through a multimode optical fibre: complex transformation analysis and applications in biophotonics},
  shorttitle = {Shaping the light transmission through a multimode optical fibre},
  author = {{\v C}i{\v z}m{\'a}r, Tom{\'a}{\v s} and Dholakia, Kishan},
  year = {2011},
  month = sep,
  volume = {19},
  pages = {18871--18884},
  publisher = {{Optical Society of America}},
  issn = {1094-4087},
  doi = {10.1364/OE.19.018871},
  journal = {Opt. Express},
  number = {20}
}

@article{cizmar2012,
  title = {Exploiting multimode waveguides for pure fibre-based imaging},
  author = {{\v C}i{\v z}m{\'a}r, Tom{\'a}{\v s} and Dholakia, Kishan},
  year = {2012},
  month = aug,
  volume = {3},
  pages = {1027},
  publisher = {{Nature Publishing Group}},
  issn = {2041-1723},
  doi = {10.1038/ncomms2024},
  journal = {Nat. Commun.},
  number = {1}
}

@article{defienne2020,
  title = {Arbitrary spatial mode sorting in a multimode fiber},
  author = {Defienne, Hugo and Faccio, Daniele},
  year = {2020},
  month = jun,
  volume = {101},
  pages = {063830},
  publisher = {{American Physical Society}},
  doi = {10.1103/PhysRevA.101.063830},
  journal = {Phys. Rev. A},
  number = {6}
}

@article{dopke2015,
  title = {Phase and amplitude calibration of dual-mask spatial light modulator for high-resolution femtosecond pulse shaping},
  author = {D{\"o}pke, B. and Balzer, J. C. and Hofmann, M. R.},
  year = {2015},
  volume = {51},
  pages = {642--644},
  issn = {0013-5194},
  doi = {10.1049/el.2015.0078},
  journal = {Electron. Lett.},
  number = {8}
}

@article{flusberg2005,
  title = {Fiber-optic fluorescence imaging},
  author = {Flusberg, Benjamin A. and Cocker, Eric D. and Piyawattanametha, Wibool and Jung, Juergen C. and Cheung, Eunice L. M. and Schnitzer, Mark J.},
  year = {2005},
  month = dec,
  volume = {2},
  pages = {941--950},
  publisher = {{Nature Publishing Group}},
  issn = {1548-7105},
  doi = {10.1038/nmeth820},
  journal = {Nat. Methods},
  number = {12}
}

@article{fu2007,
  title = {Fibre-optic nonlinear optical microscopy and endoscopy},
  author = {Fu, L. and Gu, M.},
  year = {2007},
  volume = {226},
  pages = {195--206},
  issn = {1365-2818},
  doi = {10.1111/j.1365-2818.2007.01777.x},
  annotation = {\_eprint: https://onlinelibrary.wiley.com/doi/pdf/10.1111/j.1365-2818.2007.01777.x},
  journal = {J. Microsc.},
  number = {3}
}

@article{helmchen2005,
  title = {Deep tissue two-photon microscopy},
  author = {Helmchen, Fritjof and Denk, Winfried},
  year = {2005},
  month = dec,
  volume = {2},
  pages = {932--940},
  publisher = {{Nature Publishing Group}},
  issn = {1548-7105},
  doi = {10.1038/nmeth818},
  journal = {Nat. Methods},
  number = {12}
}

@article{katz2011,
  title = {Focusing and compression of ultrashort pulses through scattering media},
  author = {Katz, Ori and Small, Eran and Bromberg, Yaron and Silberberg, Yaron},
  year = {2011},
  month = jun,
  volume = {5},
  pages = {372--377},
  issn = {1749-4893},
  doi = {10.1038/nphoton.2011.72},
  journal = {Nat. Photonics},
  number = {6}
}

@article{katz2014,
  title = {Noninvasive nonlinear focusing and imaging through strongly scattering turbid layers},
  author = {Katz, Ori and Small, Eran and Guan, Yefeng and Silberberg, Yaron},
  year = {2014},
  month = sep,
  volume = {1},
  pages = {170--174},
  publisher = {{Optical Society of America}},
  issn = {2334-2536},
  doi = {10.1364/OPTICA.1.000170},
  journal = {Optica},
  number = {3}
}

@book{kubby2019,
  title = {Wavefront {{Shaping}} for {{Biomedical Imaging}}},
  editor = {Kubby, Joel and Gigan, Sylvain and Cui, Meng},
  year = {2019},
  publisher = {{Cambridge University Press}},
  address = {{Cambridge}},
  doi = {10.1017/9781316403938},
  isbn = {978-1-107-12412-7},
  series = {Advances in {{Microscopy}} and {{Microanalysis}}}
}

@article{leonardo2011,
  title = {Hologram transmission through multi-mode optical fibers},
  author = {Leonardo, Roberto Di and Bianchi, Silvio},
  year = {2011},
  month = jan,
  volume = {19},
  pages = {247--254},
  publisher = {{Optical Society of America}},
  issn = {1094-4087},
  doi = {10.1364/OE.19.000247},
  journal = {Opt. Express},
  number = {1}
}

@article{makarov2008,
  title = {Two-photon absorption standards in the 550\textendash 1600 nm excitation wavelength range},
  author = {Makarov, Nikolay S. and Drobizhev, Mikhail and Rebane, Aleksander},
  year = {2008},
  month = mar,
  volume = {16},
  pages = {4029--4047},
  issn = {1094-4087},
  doi = {10.1364/OE.16.004029},
  journal = {Opt. Express},
  number = {6}
}

@article{mccabe2011,
  title = {Spatio-temporal focusing of an ultrafast pulse through a multiply scattering medium},
  author = {McCabe, David J. and Tajalli, Ayhan and Austin, Dane R. and Bondareff, Pierre and Walmsley, Ian A. and Gigan, Sylvain and Chatel, B{\'e}atrice},
  year = {2011},
  month = aug,
  volume = {2},
  pages = {447},
  issn = {2041-1723},
  doi = {10.1038/ncomms1434},
  journal = {Nat. Commun.}
}

@article{mezil2020,
  title = {Single-shot hybrid photoacoustic-fluorescent microendoscopy through a multimode fiber with wavefront shaping},
  author = {Mezil, Sylvain and {Caravaca-Aguirre}, Antonio M. and Zhang, Edward Z. and Moreau, Philippe and Wang, Ir{\`e}ne and Beard, Paul C. and Bossy, Emmanuel},
  year = {2020},
  month = oct,
  volume = {11},
  pages = {5717--5727},
  publisher = {{Optical Society of America}},
  issn = {2156-7085},
  doi = {10.1364/BOE.400686},
  journal = {Biomed. Opt. Express},
  number = {10}
}

@article{monmayrant2004,
  title = {New phase and amplitude high resolution pulse shaper},
  author = {Monmayrant, Antoine and Chatel, B{\'e}atrice},
  year = {2004},
  month = aug,
  volume = {75},
  pages = {2668--2671},
  issn = {0034-6748},
  doi = {10.1063/1.1771492},
  journal = {Rev. Sci. Instrum.},
  number = {8}
}

@article{morales-delgado2015a,
  title = {Two-photon imaging through a multimode fiber},
  author = {{Morales-Delgado}, Edgar E. and Psaltis, Demetri and Moser, Christophe},
  year = {2015},
  month = dec,
  volume = {23},
  pages = {32158--32170},
  publisher = {{Optical Society of America}},
  issn = {1094-4087},
  doi = {10.1364/OE.23.032158},
  journal = {Opt. Express},
  number = {25}
}

@article{morales-delgado2017,
  title = {Three-dimensional microfabrication through a multimode optical fiber},
  author = {{Morales-Delgado}, Edgar E. and Urio, Loic and Conkey, Donald B. and Stasio, Nicolino and Psaltis, Demetri and Moser, Christophe},
  year = {2017},
  month = mar,
  volume = {25},
  pages = {7031--7045},
  publisher = {{Optical Society of America}},
  issn = {1094-4087},
  doi = {10.1364/OE.25.007031},
  journal = {Opt. Express},
  number = {6}
}

@article{mounaix2019,
  title = {Control of the temporal and polarization response of a multimode fiber},
  author = {Mounaix, Mickael and Carpenter, Joel},
  year = {2019},
  month = nov,
  volume = {10},
  pages = {5085},
  publisher = {{Nature Publishing Group}},
  issn = {2041-1723},
  doi = {10.1038/s41467-019-13059-8},
  journal = {Nat. Commun.},
  number = {1}
}

@article{ngom2018,
  title = {Mode control in a multimode fiber through acquiring its transmission matrix from a reference-less optical system},
  author = {N'Gom, Moussa and Norris, Theodore B. and Michielssen, Eric and Nadakuditi, Raj Rao},
  year = {2018},
  month = feb,
  volume = {43},
  pages = {419--422},
  publisher = {{Optical Society of America}},
  issn = {1539-4794},
  doi = {10.1364/OL.43.000419},
  journal = {Opt. Lett.},
  number = {3}
}

@book{okamoto2006,
  title = {Fundamentals of {{Optical Waveguides}}},
  author = {Okamoto, Katsunari},
  year = {2006},
  edition = {second},
  publisher = {{Elsevier}},
  address = {{Amsterdam}},
  isbn = {978-0-12-525096-2},
  lccn = {TA1800 .O37 2006}
}

@article{papadopoulos2012,
  title = {Focusing and scanning light through a multimode optical fiber using digital phase conjugation},
  author = {Papadopoulos, Ioannis N. and Farahi, Salma and Moser, Christophe and Psaltis, Demetri},
  year = {2012},
  month = may,
  volume = {20},
  pages = {10583--10590},
  issn = {1094-4087},
  doi = {10.1364/OE.20.010583},
  journal = {Opt. Express},
  number = {10}
}

@article{pikalek2019,
  title = {Wavelength dependent characterization of a multimode fibre endoscope},
  author = {Pik{\'a}lek, Tom{\'a}{\v s} and Tr{\"a}g{\aa}rdh, Johanna and Simpson, Stephen and {\v C}i{\v z}m{\'a}r, Tom{\'a}{\v s}},
  year = {2019},
  month = sep,
  volume = {27},
  pages = {28239--28253},
  publisher = {{Optical Society of America}},
  issn = {1094-4087},
  doi = {10.1364/OE.27.028239},
  journal = {Opt. Express},
  number = {20}
}

@article{ploschner2015,
  title = {Seeing through chaos in multimode fibres},
  author = {Pl{\"o}schner, Martin and Tyc, Tom{\'a}{\v s} and {\v C}i{\v z}m{\'a}r, Tom{\'a}{\v s}},
  year = {2015},
  month = aug,
  volume = {9},
  pages = {529--535},
  issn = {1749-4893},
  doi = {10.1038/nphoton.2015.112},
  journal = {Nat. Photonics},
  number = {8}
}

@article{popoff2010,
  title = {Measuring the {{Transmission Matrix}} in {{Optics}}: {{An Approach}} to the {{Study}} and {{Control}} of {{Light Propagation}} in {{Disordered Media}}},
  shorttitle = {Measuring the {{Transmission Matrix}} in {{Optics}}},
  author = {Popoff, S. M. and Lerosey, G. and Carminati, R. and Fink, M. and Boccara, A. C. and Gigan, S.},
  year = {2010},
  month = mar,
  volume = {104},
  pages = {100601},
  publisher = {{American Physical Society}},
  doi = {10.1103/PhysRevLett.104.100601},
  journal = {Phys. Rev. Lett.},
  number = {10}
}

@article{popoff2011,
  title = {Controlling light through optical disordered media: transmission matrix approach},
  shorttitle = {Controlling light through optical disordered media},
  author = {Popoff, S. M. and Lerosey, G. and Fink, M. and Boccara, A. C. and Gigan, S.},
  year = {2011},
  month = dec,
  volume = {13},
  pages = {123021},
  issn = {1367-2630},
  doi = {10.1088/1367-2630/13/12/123021},
  journal = {New J. Phys.},
  number = {12}
}

@article{redding2013,
  title = {All-fiber spectrometer based on speckle pattern reconstruction},
  author = {Redding, Brandon and Popoff, Sebastien M. and Cao, Hui},
  year = {2013},
  month = mar,
  volume = {21},
  pages = {6584--6600},
  issn = {1094-4087},
  doi = {10.1364/OE.21.006584},
  journal = {Opt. Express},
  number = {5}
}

@article{rotter2017,
  title = {Light fields in complex media: {{Mesoscopic}} scattering meets wave control},
  shorttitle = {Light fields in complex media},
  author = {Rotter, Stefan and Gigan, Sylvain},
  year = {2017},
  month = mar,
  volume = {89},
  pages = {015005},
  doi = {10.1103/RevModPhys.89.015005},
  journal = {Rev. Mod. Phys.},
  number = {1}
}

@inproceedings{sutherland2016,
  title = {Characterizing octagonal and rectangular fibers for {{MAROON}}-{{X}}},
  booktitle = {Advances in {{Optical}} and {{Mechanical Technologies}} for {{Telescopes}} and {{Instrumentation II}}},
  author = {Sutherland, Adam P. and Stuermer, Julian and Miller, Katrina R. and Seifahrt, Andreas and Bean, Jacob L.},
  year = {2016},
  month = jul,
  volume = {9912},
  pages = {99125C},
  publisher = {{International Society for Optics and Photonics}},
  doi = {10.1117/12.2231707}
}

@article{tang2006,
  title = {Effect of pulse duration on two-photon excited fluorescence and second harmonic generation in nonlinear optical microscopy},
  author = {Tang, Shuo and Krasieva, Tatiana B. and Chen, Zhongping and Tempea, Gabriel and Tromberg, Bruce Jason},
  year = {2006},
  month = mar,
  volume = {11},
  pages = {020501},
  issn = {1083-3668, 1560-2281},
  doi = {10.1117/1.2177676},
  journal = {J. Biomed. Opt.},
  number = {2}
}

@article{tragardh2019,
  title = {Label-free {{CARS}} microscopy through a multimode fiber endoscope},
  author = {Tr{\"a}g{\aa}rdh, Johanna and Pik{\'a}lek, Tom{\'a}{\v s} and {\v S}er{\'y}, Mojm{\'i}r and Meyer, Tobias and Popp, J{\"u}rgen and {\v C}i{\v z}m{\'a}r, Tom{\'a}{\v s}},
  year = {2019},
  month = oct,
  volume = {27},
  pages = {30055--30066},
  publisher = {{Optical Society of America}},
  issn = {1094-4087},
  doi = {10.1364/OE.27.030055},
  journal = {Opt. Express},
  number = {21}
}

@article{turcotte2020,
  title = {Two-photon fluorescence imaging of live neurons using a multimode optical fiber},
  author = {Turcotte, Rapha{\"e}l and Schmidt, Carla C. and Booth, Martin J. and Emptage, Nigel J.},
  year = {2020},
  month = apr,
  pages = {2020.04.27.063388},
  publisher = {{Cold Spring Harbor Laboratory}},
  doi = {10.1101/2020.04.27.063388},
  chapter = {New Results},
  journal = {bioRxiv}
}

@article{turtaev2018,
  title = {High-fidelity multimode fibre-based endoscopy for deep brain in vivo imaging},
  author = {Turtaev, Sergey and Leite, Ivo T. and {Altwegg-Boussac}, Tristan and Pakan, Janelle M. P. and Rochefort, Nathalie L. and {\v C}i{\v z}m{\'a}r, Tom{\'a}{\v s}},
  year = {2018},
  month = nov,
  volume = {7},
  pages = {92},
  publisher = {{Nature Publishing Group}},
  issn = {2047-7538},
  doi = {10.1038/s41377-018-0094-x},
  journal = {Light Sci. Appl.},
  number = {1}
}

@article{vellekoop2007,
  title = {Focusing coherent light through opaque strongly scattering media},
  author = {Vellekoop, I. M. and Mosk, A. P.},
  year = {2007},
  month = aug,
  volume = {32},
  pages = {2309--2311},
  issn = {1539-4794},
  doi = {10.1364/OL.32.002309},
  journal = {Opt. Lett.},
  number = {16}
}

@article{vellekoop2008a,
  title = {Phase control algorithms for focusing light through turbid media},
  author = {Vellekoop, I. M. and Mosk, A. P.},
  year = {2008},
  month = jun,
  volume = {281},
  pages = {3071--3080},
  issn = {0030-4018},
  doi = {10.1016/j.optcom.2008.02.022},
  journal = {Opt. Commun.},
  number = {11}
}

@article{vellekoop2015,
  title = {Feedback-based wavefront shaping},
  author = {Vellekoop, Ivo M.},
  year = {2015},
  month = may,
  volume = {23},
  pages = {12189--12206},
  issn = {1094-4087},
  doi = {10.1364/OE.23.012189},
  journal = {Opt. Express},
  number = {9}
}

@article{xiong2016,
  title = {Spatiotemporal {{Control}} of {{Light Transmission}} through a {{Multimode Fiber}} with {{Strong Mode Coupling}}},
  author = {Xiong, Wen and Ambichl, Philipp and Bromberg, Yaron and Redding, Brandon and Rotter, Stefan and Cao, Hui},
  year = {2016},
  month = jul,
  volume = {117},
  pages = {053901},
  doi = {10.1103/PhysRevLett.117.053901},
  journal = {Phys. Rev. Lett.},
  number = {5}
}

@article{xiong2019,
  title = {Long-range spatio-temporal correlations in multimode fibers for pulse delivery},
  author = {Xiong, Wen and Hsu, Chia Wei and Cao, Hui},
  year = {2019},
  month = jul,
  volume = {10},
  pages = {2973},
  issn = {2041-1723},
  doi = {10.1038/s41467-019-10916-4},
  journal = {Nat. Commun.},
  number = {1}
}




==> tWFS_Velsink2.tex <==
@article{amitonova2016,
  title = {High-resolution wavefront shaping with a photonic crystal fiber for multimode fiber imaging},
  author = {Amitonova, Lyubov V. and Descloux, Adrien and Petschulat, Joerg and Frosz, Michael H. and Ahmed, Goran and Babic, Fehim and Jiang, Xin and Mosk, Allard P. and Russell, Philip St J. and Pinkse, Pepijn W. H.},
  year = {2016},
  month = feb,
  volume = {41},
  pages = {497--500},
  publisher = {{Optical Society of America}},
  issn = {1539-4794},
  doi = {10.1364/OL.41.000497},
  journal = {Opt. Lett.},
  number = {3}
}

@article{amitonova2020,
  title = {Endo-microscopy beyond the {{Abbe}} and {{Nyquist}} limits},
  author = {Amitonova, Lyubov V. and {de Boer}, Johannes F.},
  year = {2020},
  month = may,
  volume = {9},
  pages = {81},
  publisher = {{Nature Publishing Group}},
  issn = {2047-7538},
  doi = {10.1038/s41377-020-0308-x},
  journal = {Light Sci. Appl.},
  number = {1}
}

@article{andresen2013,
  title = {Toward endoscopes with no distal optics: video-rate scanning microscopy through a fiber bundle},
  shorttitle = {Toward endoscopes with no distal optics},
  author = {Andresen, Esben Ravn and Bouwmans, G{\'e}raud and Monneret, Serge and Rigneault, Herv{\'e}},
  year = {2013},
  month = mar,
  volume = {38},
  pages = {609--611},
  publisher = {{Optical Society of America}},
  issn = {1539-4794},
  doi = {10.1364/OL.38.000609},
  journal = {Opt. Lett.},
  number = {5}
}

@article{borhani2018,
  title = {Learning to see through multimode fibers},
  author = {Borhani, Navid and Kakkava, Eirini and Moser, Christophe and Psaltis, Demetri},
  year = {2018},
  month = aug,
  volume = {5},
  pages = {960--966},
  publisher = {{Optical Society of America}},
  issn = {2334-2536},
  doi = {10.1364/OPTICA.5.000960},
  journal = {Optica},
  number = {8}
}

@article{bowlan2006,
  title = {Crossed-beam spectral interferometry: a simple, high-spectral-resolution method for completely characterizing complex ultrashort pulses in real time},
  shorttitle = {Crossed-beam spectral interferometry},
  author = {Bowlan, Pamela and Gabolde, Pablo and Shreenath, Aparna and McGresham, Kristan and Trebino, Rick and Akturk, Selcuk},
  year = {2006},
  month = nov,
  volume = {14},
  pages = {11892--11900},
  publisher = {{Optical Society of America}},
  issn = {1094-4087},
  doi = {10.1364/OE.14.011892},
  journal = {Opt. Express},
  number = {24}
}

@article{cizmar2011,
  title = {Shaping the light transmission through a multimode optical fibre: complex transformation analysis and applications in biophotonics},
  shorttitle = {Shaping the light transmission through a multimode optical fibre},
  author = {{\v C}i{\v z}m{\'a}r, Tom{\'a}{\v s} and Dholakia, Kishan},
  year = {2011},
  month = sep,
  volume = {19},
  pages = {18871--18884},
  publisher = {{Optical Society of America}},
  issn = {1094-4087},
  doi = {10.1364/OE.19.018871},
  journal = {Opt. Express},
  number = {20}
}

@article{cizmar2012,
  title = {Exploiting multimode waveguides for pure fibre-based imaging},
  author = {{\v C}i{\v z}m{\'a}r, Tom{\'a}{\v s} and Dholakia, Kishan},
  year = {2012},
  month = aug,
  volume = {3},
  pages = {1027},
  publisher = {{Nature Publishing Group}},
  issn = {2041-1723},
  doi = {10.1038/ncomms2024},
  journal = {Nat. Commun.},
  number = {1}
}

@article{defienne2020,
  title = {Arbitrary spatial mode sorting in a multimode fiber},
  author = {Defienne, Hugo and Faccio, Daniele},
  year = {2020},
  month = jun,
  volume = {101},
  pages = {063830},
  publisher = {{American Physical Society}},
  doi = {10.1103/PhysRevA.101.063830},
  journal = {Phys. Rev. A},
  number = {6}
}

@article{dopke2015,
  title = {Phase and amplitude calibration of dual-mask spatial light modulator for high-resolution femtosecond pulse shaping},
  author = {D{\"o}pke, B. and Balzer, J. C. and Hofmann, M. R.},
  year = {2015},
  volume = {51},
  pages = {642--644},
  issn = {0013-5194},
  doi = {10.1049/el.2015.0078},
  journal = {Electron. Lett.},
  number = {8}
}

@article{flusberg2005,
  title = {Fiber-optic fluorescence imaging},
  author = {Flusberg, Benjamin A. and Cocker, Eric D. and Piyawattanametha, Wibool and Jung, Juergen C. and Cheung, Eunice L. M. and Schnitzer, Mark J.},
  year = {2005},
  month = dec,
  volume = {2},
  pages = {941--950},
  publisher = {{Nature Publishing Group}},
  issn = {1548-7105},
  doi = {10.1038/nmeth820},
  journal = {Nat. Methods},
  number = {12}
}

@article{fu2007,
  title = {Fibre-optic nonlinear optical microscopy and endoscopy},
  author = {Fu, L. and Gu, M.},
  year = {2007},
  volume = {226},
  pages = {195--206},
  issn = {1365-2818},
  doi = {10.1111/j.1365-2818.2007.01777.x},
  annotation = {\_eprint: https://onlinelibrary.wiley.com/doi/pdf/10.1111/j.1365-2818.2007.01777.x},
  journal = {J. Microsc.},
  number = {3}
}

@article{helmchen2005,
  title = {Deep tissue two-photon microscopy},
  author = {Helmchen, Fritjof and Denk, Winfried},
  year = {2005},
  month = dec,
  volume = {2},
  pages = {932--940},
  publisher = {{Nature Publishing Group}},
  issn = {1548-7105},
  doi = {10.1038/nmeth818},
  journal = {Nat. Methods},
  number = {12}
}

@article{katz2011,
  title = {Focusing and compression of ultrashort pulses through scattering media},
  author = {Katz, Ori and Small, Eran and Bromberg, Yaron and Silberberg, Yaron},
  year = {2011},
  month = jun,
  volume = {5},
  pages = {372--377},
  issn = {1749-4893},
  doi = {10.1038/nphoton.2011.72},
  journal = {Nat. Photonics},
  number = {6}
}

@article{katz2014,
  title = {Noninvasive nonlinear focusing and imaging through strongly scattering turbid layers},
  author = {Katz, Ori and Small, Eran and Guan, Yefeng and Silberberg, Yaron},
  year = {2014},
  month = sep,
  volume = {1},
  pages = {170--174},
  publisher = {{Optical Society of America}},
  issn = {2334-2536},
  doi = {10.1364/OPTICA.1.000170},
  journal = {Optica},
  number = {3}
}

@book{kubby2019,
  title = {Wavefront {{Shaping}} for {{Biomedical Imaging}}},
  editor = {Kubby, Joel and Gigan, Sylvain and Cui, Meng},
  year = {2019},
  publisher = {{Cambridge University Press}},
  address = {{Cambridge}},
  doi = {10.1017/9781316403938},
  isbn = {978-1-107-12412-7},
  series = {Advances in {{Microscopy}} and {{Microanalysis}}}
}

@article{leonardo2011,
  title = {Hologram transmission through multi-mode optical fibers},
  author = {Leonardo, Roberto Di and Bianchi, Silvio},
  year = {2011},
  month = jan,
  volume = {19},
  pages = {247--254},
  publisher = {{Optical Society of America}},
  issn = {1094-4087},
  doi = {10.1364/OE.19.000247},
  journal = {Opt. Express},
  number = {1}
}

@article{makarov2008,
  title = {Two-photon absorption standards in the 550\textendash 1600 nm excitation wavelength range},
  author = {Makarov, Nikolay S. and Drobizhev, Mikhail and Rebane, Aleksander},
  year = {2008},
  month = mar,
  volume = {16},
  pages = {4029--4047},
  issn = {1094-4087},
  doi = {10.1364/OE.16.004029},
  journal = {Opt. Express},
  number = {6}
}

@article{mccabe2011,
  title = {Spatio-temporal focusing of an ultrafast pulse through a multiply scattering medium},
  author = {McCabe, David J. and Tajalli, Ayhan and Austin, Dane R. and Bondareff, Pierre and Walmsley, Ian A. and Gigan, Sylvain and Chatel, B{\'e}atrice},
  year = {2011},
  month = aug,
  volume = {2},
  pages = {447},
  issn = {2041-1723},
  doi = {10.1038/ncomms1434},
  journal = {Nat. Commun.}
}

@article{mezil2020,
  title = {Single-shot hybrid photoacoustic-fluorescent microendoscopy through a multimode fiber with wavefront shaping},
  author = {Mezil, Sylvain and {Caravaca-Aguirre}, Antonio M. and Zhang, Edward Z. and Moreau, Philippe and Wang, Ir{\`e}ne and Beard, Paul C. and Bossy, Emmanuel},
  year = {2020},
  month = oct,
  volume = {11},
  pages = {5717--5727},
  publisher = {{Optical Society of America}},
  issn = {2156-7085},
  doi = {10.1364/BOE.400686},
  journal = {Biomed. Opt. Express},
  number = {10}
}

@article{monmayrant2004,
  title = {New phase and amplitude high resolution pulse shaper},
  author = {Monmayrant, Antoine and Chatel, B{\'e}atrice},
  year = {2004},
  month = aug,
  volume = {75},
  pages = {2668--2671},
  issn = {0034-6748},
  doi = {10.1063/1.1771492},
  journal = {Rev. Sci. Instrum.},
  number = {8}
}

@article{morales-delgado2015a,
  title = {Two-photon imaging through a multimode fiber},
  author = {{Morales-Delgado}, Edgar E. and Psaltis, Demetri and Moser, Christophe},
  year = {2015},
  month = dec,
  volume = {23},
  pages = {32158--32170},
  publisher = {{Optical Society of America}},
  issn = {1094-4087},
  doi = {10.1364/OE.23.032158},
  journal = {Opt. Express},
  number = {25}
}

@article{morales-delgado2017,
  title = {Three-dimensional microfabrication through a multimode optical fiber},
  author = {{Morales-Delgado}, Edgar E. and Urio, Loic and Conkey, Donald B. and Stasio, Nicolino and Psaltis, Demetri and Moser, Christophe},
  year = {2017},
  month = mar,
  volume = {25},
  pages = {7031--7045},
  publisher = {{Optical Society of America}},
  issn = {1094-4087},
  doi = {10.1364/OE.25.007031},
  journal = {Opt. Express},
  number = {6}
}

@article{mounaix2019,
  title = {Control of the temporal and polarization response of a multimode fiber},
  author = {Mounaix, Mickael and Carpenter, Joel},
  year = {2019},
  month = nov,
  volume = {10},
  pages = {5085},
  publisher = {{Nature Publishing Group}},
  issn = {2041-1723},
  doi = {10.1038/s41467-019-13059-8},
  journal = {Nat. Commun.},
  number = {1}
}

@article{ngom2018,
  title = {Mode control in a multimode fiber through acquiring its transmission matrix from a reference-less optical system},
  author = {N'Gom, Moussa and Norris, Theodore B. and Michielssen, Eric and Nadakuditi, Raj Rao},
  year = {2018},
  month = feb,
  volume = {43},
  pages = {419--422},
  publisher = {{Optical Society of America}},
  issn = {1539-4794},
  doi = {10.1364/OL.43.000419},
  journal = {Opt. Lett.},
  number = {3}
}

@book{okamoto2006,
  title = {Fundamentals of {{Optical Waveguides}}},
  author = {Okamoto, Katsunari},
  year = {2006},
  edition = {second},
  publisher = {{Elsevier}},
  address = {{Amsterdam}},
  isbn = {978-0-12-525096-2},
  lccn = {TA1800 .O37 2006}
}

@article{papadopoulos2012,
  title = {Focusing and scanning light through a multimode optical fiber using digital phase conjugation},
  author = {Papadopoulos, Ioannis N. and Farahi, Salma and Moser, Christophe and Psaltis, Demetri},
  year = {2012},
  month = may,
  volume = {20},
  pages = {10583--10590},
  issn = {1094-4087},
  doi = {10.1364/OE.20.010583},
  journal = {Opt. Express},
  number = {10}
}

@article{pikalek2019,
  title = {Wavelength dependent characterization of a multimode fibre endoscope},
  author = {Pik{\'a}lek, Tom{\'a}{\v s} and Tr{\"a}g{\aa}rdh, Johanna and Simpson, Stephen and {\v C}i{\v z}m{\'a}r, Tom{\'a}{\v s}},
  year = {2019},
  month = sep,
  volume = {27},
  pages = {28239--28253},
  publisher = {{Optical Society of America}},
  issn = {1094-4087},
  doi = {10.1364/OE.27.028239},
  journal = {Opt. Express},
  number = {20}
}

@article{ploschner2015,
  title = {Seeing through chaos in multimode fibres},
  author = {Pl{\"o}schner, Martin and Tyc, Tom{\'a}{\v s} and {\v C}i{\v z}m{\'a}r, Tom{\'a}{\v s}},
  year = {2015},
  month = aug,
  volume = {9},
  pages = {529--535},
  issn = {1749-4893},
  doi = {10.1038/nphoton.2015.112},
  journal = {Nat. Photonics},
  number = {8}
}

@article{popoff2010,
  title = {Measuring the {{Transmission Matrix}} in {{Optics}}: {{An Approach}} to the {{Study}} and {{Control}} of {{Light Propagation}} in {{Disordered Media}}},
  shorttitle = {Measuring the {{Transmission Matrix}} in {{Optics}}},
  author = {Popoff, S. M. and Lerosey, G. and Carminati, R. and Fink, M. and Boccara, A. C. and Gigan, S.},
  year = {2010},
  month = mar,
  volume = {104},
  pages = {100601},
  publisher = {{American Physical Society}},
  doi = {10.1103/PhysRevLett.104.100601},
  journal = {Phys. Rev. Lett.},
  number = {10}
}

@article{popoff2011,
  title = {Controlling light through optical disordered media: transmission matrix approach},
  shorttitle = {Controlling light through optical disordered media},
  author = {Popoff, S. M. and Lerosey, G. and Fink, M. and Boccara, A. C. and Gigan, S.},
  year = {2011},
  month = dec,
  volume = {13},
  pages = {123021},
  issn = {1367-2630},
  doi = {10.1088/1367-2630/13/12/123021},
  journal = {New J. Phys.},
  number = {12}
}

@article{redding2013,
  title = {All-fiber spectrometer based on speckle pattern reconstruction},
  author = {Redding, Brandon and Popoff, Sebastien M. and Cao, Hui},
  year = {2013},
  month = mar,
  volume = {21},
  pages = {6584--6600},
  issn = {1094-4087},
  doi = {10.1364/OE.21.006584},
  journal = {Opt. Express},
  number = {5}
}

@article{rotter2017,
  title = {Light fields in complex media: {{Mesoscopic}} scattering meets wave control},
  shorttitle = {Light fields in complex media},
  author = {Rotter, Stefan and Gigan, Sylvain},
  year = {2017},
  month = mar,
  volume = {89},
  pages = {015005},
  doi = {10.1103/RevModPhys.89.015005},
  journal = {Rev. Mod. Phys.},
  number = {1}
}

@inproceedings{sutherland2016,
  title = {Characterizing octagonal and rectangular fibers for {{MAROON}}-{{X}}},
  booktitle = {Advances in {{Optical}} and {{Mechanical Technologies}} for {{Telescopes}} and {{Instrumentation II}}},
  author = {Sutherland, Adam P. and Stuermer, Julian and Miller, Katrina R. and Seifahrt, Andreas and Bean, Jacob L.},
  year = {2016},
  month = jul,
  volume = {9912},
  pages = {99125C},
  publisher = {{International Society for Optics and Photonics}},
  doi = {10.1117/12.2231707}
}

@article{tang2006,
  title = {Effect of pulse duration on two-photon excited fluorescence and second harmonic generation in nonlinear optical microscopy},
  author = {Tang, Shuo and Krasieva, Tatiana B. and Chen, Zhongping and Tempea, Gabriel and Tromberg, Bruce Jason},
  year = {2006},
  month = mar,
  volume = {11},
  pages = {020501},
  issn = {1083-3668, 1560-2281},
  doi = {10.1117/1.2177676},
  journal = {J. Biomed. Opt.},
  number = {2}
}

@article{tragardh2019,
  title = {Label-free {{CARS}} microscopy through a multimode fiber endoscope},
  author = {Tr{\"a}g{\aa}rdh, Johanna and Pik{\'a}lek, Tom{\'a}{\v s} and {\v S}er{\'y}, Mojm{\'i}r and Meyer, Tobias and Popp, J{\"u}rgen and {\v C}i{\v z}m{\'a}r, Tom{\'a}{\v s}},
  year = {2019},
  month = oct,
  volume = {27},
  pages = {30055--30066},
  publisher = {{Optical Society of America}},
  issn = {1094-4087},
  doi = {10.1364/OE.27.030055},
  journal = {Opt. Express},
  number = {21}
}

@article{turcotte2020,
  title = {Two-photon fluorescence imaging of live neurons using a multimode optical fiber},
  author = {Turcotte, Rapha{\"e}l and Schmidt, Carla C. and Booth, Martin J. and Emptage, Nigel J.},
  year = {2020},
  month = apr,
  pages = {2020.04.27.063388},
  publisher = {{Cold Spring Harbor Laboratory}},
  doi = {10.1101/2020.04.27.063388},
  chapter = {New Results},
  journal = {bioRxiv}
}

@article{turtaev2018,
  title = {High-fidelity multimode fibre-based endoscopy for deep brain in vivo imaging},
  author = {Turtaev, Sergey and Leite, Ivo T. and {Altwegg-Boussac}, Tristan and Pakan, Janelle M. P. and Rochefort, Nathalie L. and {\v C}i{\v z}m{\'a}r, Tom{\'a}{\v s}},
  year = {2018},
  month = nov,
  volume = {7},
  pages = {92},
  publisher = {{Nature Publishing Group}},
  issn = {2047-7538},
  doi = {10.1038/s41377-018-0094-x},
  journal = {Light Sci. Appl.},
  number = {1}
}

@article{vellekoop2007,
  title = {Focusing coherent light through opaque strongly scattering media},
  author = {Vellekoop, I. M. and Mosk, A. P.},
  year = {2007},
  month = aug,
  volume = {32},
  pages = {2309--2311},
  issn = {1539-4794},
  doi = {10.1364/OL.32.002309},
  journal = {Opt. Lett.},
  number = {16}
}

@article{vellekoop2008a,
  title = {Phase control algorithms for focusing light through turbid media},
  author = {Vellekoop, I. M. and Mosk, A. P.},
  year = {2008},
  month = jun,
  volume = {281},
  pages = {3071--3080},
  issn = {0030-4018},
  doi = {10.1016/j.optcom.2008.02.022},
  journal = {Opt. Commun.},
  number = {11}
}

@article{vellekoop2015,
  title = {Feedback-based wavefront shaping},
  author = {Vellekoop, Ivo M.},
  year = {2015},
  month = may,
  volume = {23},
  pages = {12189--12206},
  issn = {1094-4087},
  doi = {10.1364/OE.23.012189},
  journal = {Opt. Express},
  number = {9}
}

@article{xiong2016,
  title = {Spatiotemporal {{Control}} of {{Light Transmission}} through a {{Multimode Fiber}} with {{Strong Mode Coupling}}},
  author = {Xiong, Wen and Ambichl, Philipp and Bromberg, Yaron and Redding, Brandon and Rotter, Stefan and Cao, Hui},
  year = {2016},
  month = jul,
  volume = {117},
  pages = {053901},
  doi = {10.1103/PhysRevLett.117.053901},
  journal = {Phys. Rev. Lett.},
  number = {5}
}

@article{xiong2019,
  title = {Long-range spatio-temporal correlations in multimode fibers for pulse delivery},
  author = {Xiong, Wen and Hsu, Chia Wei and Cao, Hui},
  year = {2019},
  month = jul,
  volume = {10},
  pages = {2973},
  issn = {2041-1723},
  doi = {10.1038/s41467-019-10916-4},
  journal = {Nat. Commun.},
  number = {1}
}



